FQuAD: French Question Answering Dataset

Recent advances in the field of language modeling have improved state-of-the-art results on many Natural Language Processing tasks. Among them, Reading Comprehension has made significant progress over the past few years. However, most results are reported in English since labeled resources available in other languages, such as French, remain scarce. In the present work, we introduce the French Question Answering Dataset (FQuAD). FQuAD is a French Native Reading Comprehension dataset of questions and answers on a set of Wikipedia articles that consists of 25,000+ samples for the 1.0 version and 60,000+ samples for the 1.1 version. We train a baseline model which achieves an F1 score of 92.2 and an exact match ratio of 82.1 on the test set. In order to track the progress of French Question Answering models we propose a leader-board and we have made the 1.0 version of our dataset freely available at https://illuin-tech.github.io/FQuAD-explorer/.

==> content/approach.tex <==
First, we develop a native French Question Answering dataset that is similar to SQuAD1.1 \citeauthor{rajpurkar-etal-2016-squad} and we follow the same guidelines as theirs.
Indeed, while other Reading Comprehension datasets exists, many efforts have been carried out into translating SQuAD, such as in Spanish by \citeauthor{spanishsquad} or into building  Cross-lingual evaluation benchmarks \cite{mlqa} for other languages but not French.

Second, we French Question Answering model is trained by fine-tuning CamemBERT\cite{camembert} and FlauBERT\cite{camembert} on FQuAD and on the translated dataset.
\textcolor{red}{parler des modèles multilingues ? garder le paragraphe présentant l'approche sur la traduction ?}

Third, since no French Reading Comprehension dataset is currently available we translate SQuAD1.1 into French with the English-French NMT model (\citeauthor{french-nmt}, \citeyear{french-nmt}). 
As it is still not clear how the translation process affects the performances on native datasets, we compare the results for both approaches.
Translation based approaches face the challenging issue of aligning source and translated pieces of text, as the words order and quantity may change during translation. Although realignment difficulties deprived us from approximately half of the original dataset, 40,000 samples were still collected. Training an adapted CamemBERT (\citeauthor{camembert}) model for QA on this translated SQuAD1.1. Results of this training are presented in the Experiments section.
